On the Post-Lie Structure in SISO Affine Feedback Control Systems

The main objective of this work is to show that the single-input, single-output (SISO) affine feedback group, a transformation group in the context of the affine feedback interconnection of Chen-Fliess series, is a post-group in the sense of Bai, Guo, Sheng and Tang.

==> sticks-and-cups.tex <==
\tikzset{
  ncone/.pic={
	\draw (0,0)--(0,0.2);
  }
}

\tikzset{
  nctwo/.pic={
    \draw (0,0)--(0,0.2);
	\draw (0.1,0)--(0.1,0.2);
  }
}

\tikzset{
  nctwoW/.pic={
    \draw (0,0.2)--(0,0)--(0.1,0)--(0.1,0.2);
  }
}

\tikzset{
  nctwoWW/.pic={
    \draw (0,0.2)--(0,0)--(0.2,0)--(0.2,0.2);
  }
}

\tikzset{
  ncthreeWW/.pic={
    \draw (0,0.2)--(0,0)--(0.3,0)--(0.3,0.2);
	\draw (0.2,0)--(0.2,0.2);
  }
}

\tikzset{
  ncthree/.pic={
    \draw (0,0)--(0,0.2);
	\draw (0.1,0)--(0.1,0.2);
	\draw (0.2,0)--(0.2,0.2);
  }
}

\tikzset{
  ncthreeW/.pic={
    \draw (0,0.2)--(0,0)--(0.2,0)--(0.2,0.2);
	\draw (0.1,0)--(0.1,0.2);
  }
}

\tikzset{
  ncfour/.pic={
    \draw (0,0)--(0,0.2);
	\draw (0.1,0)--(0.1,0.2);
	\draw (0.2,0)--(0.2,0.2);
	\draw (0.3,0)--(0.3,0.2);
  }
}
\tikzset{
  ncfive/.pic={
    \draw (0,0)--(0,0.2);
	\draw (0.1,0)--(0.1,0.2);
	\draw (0.2,0)--(0.2,0.2);
	\draw (0.3,0)--(0.3,0.2);
	\draw (0.4,0)--(0.4,0.2);
  }
}


\tikzset{
  ncfourW/.pic={
    \draw (0,0.2)--(0,0)--(0.3,0)--(0.3,0.2);
	\draw (0.1,0)--(0.1,0.2);
	\draw (0.2,0)--(0.2,0.2);
  }
}
\tikzset{
  ncfiveW/.pic={
    \draw (0,0.2)--(0,0)--(0.4,0)--(0.4,0.2);
	\draw (0.1,0)--(0.1,0.2);
	\draw (0.2,0)--(0.2,0.2);
	\draw (0.3,0)--(0.3,0.2);
  }
}

\tikzset{
  nconeinsidetwoWW/.pic={
    \path (0,0) pic {nctwoWW}; \path (0.1,0.1) pic {ncone};
  }
}

\tikzset{
  nconeinsidethreeWW/.pic={
    \path (0,0) pic {ncthreeWW}; \path (0.1,0.1) pic {ncone};
  }
}
\tikzset{
  nconeinsidethreerightWW/.pic={
    \draw (0,0.2)--(0,0)--(0.3,0)--(0.3,0.2);
    \draw (0.1,0)--(0.1,0.2); \draw (0.2,0.1)--(0.2,0.3);
  }
}
\tikzset{
  nconeinsidethreeleftWW/.pic={
    \draw (0,0.2)--(0,0)--(0.3,0)--(0.3,0.2);
    \draw (0.2,0)--(0.2,0.2); \draw (0.1,0.1)--(0.1,0.3);
  }
}
\tikzset{
  nctwoWWW/.pic={
    \draw (0,0.2)--(0,0)--(0.3,0)--(0.3,0.2);
  }
}

\tikzset{
  nconeoneinsidetwoWW/.pic={
	\path (0,0) pic {ncone};
    \path (0.1,0) pic {nctwoWW}; 
	\path (0.2,0.1) pic {ncone};
  }
}



\newcommand{\ncone}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {ncone}}\,}
\newcommand{\nctwo}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {nctwo}}\,}
\newcommand{\nctwoW}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {nctwoW}}\,}
\newcommand{\nctwoWW}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {nctwoWW}}\,}
\newcommand{\ncthree}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {ncthree}}\,}
\newcommand{\ncthreeW}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {ncthreeW}}\,}
\newcommand{\ncfour}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {ncfour}}\,}
\newcommand{\ncfive}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {ncfive}}\,}
\newcommand{\ncfourW}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {ncfourW}}\,}
\newcommand{\ncfiveW}{\,\tikz[x=1.3cm,y=1.3cm]{\path (0,0) pic {ncfiveW}}\,}
\newcommand{\nconeinsidetwoWW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nconeinsidetwoWW};
}\,}
\newcommand{\nconetwoW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {ncone}; \path (0.1,0) pic {nctwoW};
}\,}
\newcommand{\nctwoWone}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nctwoW}; \path (0.2,0) pic {ncone};
}\,}
\newcommand{\nctwoWtwoW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nctwoW}; \path (0.2,0) pic {nctwoW};
}\,}
\newcommand{\nctwoWinsidetwoWWW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nctwoWWW}; \path (0.1,0.1) pic {nctwoW};
}\,}
\newcommand{\nconeonetwoW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {ncone}; \path (0.1,0) pic {ncone}; \path (0.2,0) pic {nctwoW};
}\,}


\newcommand{\nconethreeW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {ncone}; \path (0.1,0) pic {ncthreeW};
}\,}


\newcommand{\nconeinsidethreeWW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nconeinsidethreeWW};
}\,}
\newcommand{\nconeinsidethreerightWW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nconeinsidethreerightWW};
}\,}
\newcommand{\nconeinsidethreeleftWW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nconeinsidethreeleftWW};
}\,}

\newcommand{\nconeoneinsidetwoWW}{\,\tikz[x=1.3cm,y=1.3cm]{
  \path (0,0) pic {nconeoneinsidetwoWW};
}\,}


